A Survey of Modern Compiler Fuzzing

Most software that runs on computers undergoes processing by compilers. Since compilers constitute the fundamental infrastructure of software development, their correctness is paramount. Over the years, researchers have invested in analyzing, understanding, and characterizing the bug features over mainstream compilers. These studies have demonstrated that compilers correctness requires greater research attention, and they also pave the way for compiler fuzzing. To improve compilers correctness, researchers have proposed numerous compiler fuzzing techniques. These techniques were initially developed for testing traditional compilers such as GCC/LLVM and have since been generalized to test various newly developed, domain-specific compilers, such as graphics shader compilers and deep learning (DL) compilers. In this survey, we provide a comprehensive summary of the research efforts for understanding and addressing compilers defects. Specifically, this survey mainly covers two aspects. First, it covers researchers investigation and expertise on compilers bugs, such as their symptoms and root causes. The compiler bug studies cover GCC/LLVM, JVM compilers, and DL compilers. In addition, it covers researchers efforts in designing fuzzing techniques, including constructing test programs and designing test oracles. Besides discussing the existing work, this survey outlines several open challenges and highlights research opportunities.

==> debug.tex <==
\section{Compiler Debugging}
\label{sec: Compiler Debugging}

Once the above-mentioned testing techniques produce bug-revealing test programs, 
developers begin to identify, understand, locate, and fix the bug.
These steps are together interpreted as debugging~\cite{10.5555/1077048}. 
However, several real-life problems prevent efficient debugging.
\begin{itemize}
  \item The test program constructors (Section \ref{sec:Test Program Construction Approaches})
        can produce a large number of bug-triggering test programs in just one night.
        And commonly, many test programs trigger the same compiler bug.
        Analyzing these redundant test programs can be a frustrating and time-consuming task
        for developers.
  \item The test program constructors (Section \ref{sec:Test Program Construction Approaches})
        tend to generate large test programs.
        For instance,
        the test programs generated by \textit{Csmith}~\cite{Csmith}
        is 81 KB on average~\cite{CReducer}.
        Comprehending the cause of a bug can be challenging
        for developers due to the large size of test programs.
  \item Before fixing the bug with expertise, developers need to isolate the suspicious source
        files related to the bug. However, the isolation is challenging due to the complexity of
        real-life compilers.
\end{itemize}
In this section, I arrange the contents into three sections, each corresponding
to the solution to one problem in order.


\subsection{Test Program Reduction}
\label{sec: Test Program Reduction}
Test programs generated by automated testing techniques tend to be significant in size,
complicating the developers' analysis of bugs' triggering conditions and root causes.
Therefore, the first step to address this issue is reducing the size of the test programs.

\myparagraph{Algorithms}
Zeller~\cite{deltadebugging} proposes the delta debugging prototype for narrowing down failure-inducing circumstances until a minimal set remains.
This prototype has inspired several research efforts to adjust it for reducing the size of test programs in compiler testing.
For instance,
Zeller et al.~\cite{ddmin} propose minimizing delta debugging algorithm (\textit{ddmin}), 
which can reduce the size of the test programs to the possible minimum while retaining its bug-revealing ability.
Specifically, \textit{ddmin} can remove a substring from the source code in each iteration and repeat this step until no removable substring can be found.
However, test programs are always hierarchical (\eg C source programs can be interpreted as an abstract syntax tree) and \textit{ddmin} ignores the information behind the hierarchy.
To utilize this information and achieve more efficient automated delta debugging, 
Misherghi et al.~\cite{HDD} propose hierarchical delta debugging (\textit{HDD}).
As for reducing C programs, \textit{HDD} can first parse it into an abstract syntax tree (AST) and attempts to exclude a whole subtree from the AST.
If removing a subtree causes another compilation failure or eliminates the original compilation failure, \textit{HDD} will move on to a smaller subtree to repeat the exclusion attempt.
\textit{HDD} can recursively perform the above two steps until finding the biggest removable subtree unrelated to the original failure.
In this way, \textit{HDD} is bolder in test program reduction and thus more efficient than \textit{ddmin}.
Besides,
Wang et al.~\cite{ProbDD} argue that \textit{ddmin} fails to utilize the information from existing test results.
Therefore \textit{ddmin} cannot obtain minimized test programs.
To this end, they
propose a probabilistic delta debugging algorithm (named \textit{ProbDD}) to
train a probabilistic model to estimate the probabilities for the elements to be kept
in the reduced test programs.
They perform experiments on GCC bugs and Clang bugs, prove the correctness of \textit{ProbDD} and demonstrate its ability in size reduction.
Delta debugging algorithms have been evolving towards being faster and making the test programs slimmer. 

\myparagraph{Techniques}
In addition to improvements to the algorithm, researchers also investigate better utilizing these algorithms for real-life tasks.
Groce et al.~\cite{causereduction} argue that \textit{ddmin} reduces the size of the test programs so much that the reduction may trigger information loss, which is not good for test efficiency.
Therefore, they
introduce \textit{cause reduction}, an extension of delta debugging,
to reduce the size of test programs while retaining the code coverage.
Regehr et al.~\cite{CReducer} argue that the proposed delta debugging algorithms are not well-suited for reducing real-life C programs due to the following factors:
\begin{itemize}
  \item These algorithms do not contain rich transformation strategies such as removing a parameter from a function and the corresponding argument of its call sites, which are required for real-life reduction tasks.
  \item These algorithms are greedy and may fall into local minima and output programs that are not small enough in size.
  \item These algorithms cannot promise the validity of the reduced programs.
  \item These algorithms tend to generate tiny but not readable test programs (This argument is similar to that of Groce's).
\end{itemize}
To resolve these problems, they propose three C program reducers, two of which can only reduce Csmith-generated C programs while the remaining one can reduce any C programs.
The most efficient reducer of the three, \textit{C-Reduce}, can reduce general C programs and generate reduced programs that are smaller than the programs generated by the other two over 25X on average.
And the experimental results show that \textit{C-Reduce} can generate much smaller test programs with a similar time cost to that of a general delta debugging algorithm.
The success of \textit{C-Reduce} also inspires similar research efforts on OpenCL~\cite{10.1145/2909437.2909439}.
Though C-Reduce is provably efficient in test program reduction, it requires dynamic analysis tools (\eg Clang Static Analyzer\footnote{\url{https://clang.llvm.org/docs/ClangStaticAnalyzer.html}}, AddressSanitizer\footnote{\url{https://clang.llvm.org/docs/AddressSanitizer.html}}, and MemorySanitizer\footnote{\url{https://clang.llvm.org/docs/MemorySanitizer.html}})
to monitor the reduction process and discard UB-contained reduced programs.
The utilization of these tools makes \textit{C-Reduce} dependent, bug-prone (since these tools may be imprecise) and expensive.
To solve this problem, Donaldson~\cite{spirv-fuzz} attempts almost-free test program reduction by designing transformations in the following principles.
\begin{itemize}
  \item Maximize independence among transformations. This principle eases the difficulty of deleting a transformation that has dependants from a transformation sequence.
  \item Favor simple transformation and try to make transformation atomic. This principle breaks down a conceptually large transformation into atomic and small ones and can help locate the bug-triggered small transformation.
\end{itemize}
With these two principles, test program reduction is free of heavy-handed tools.
Until now, the delta-debugging algorithms and the related techniques all focus on the single file. 
However, interdependent code files are common in reality. The reduction of these files without breaking the interdependence is still a challenge.
To address this issue, Le el al.~\cite{Proteus} propose \textit{Split} to reduce multiple code files generated by their proposed technique \textit{Proteus}.
Specifically, \textit{Proteus} can break a code file into multiple interdependent files and test link-time optimizations with these files.
After detecting a bug, \textit{Split} can first perform delta debugging on the original single code file and split the reduced version of the code into multiple code files.
After each reduction step, \textit{Split} checks for the existence of the bug-triggering behavior.



Reducing a single test program or several interdependent test programs 
